Towards Seamless Authentication for Zoom-Based Online Teaching and Meeting

The lockdowns and travel restrictions in current coronavirus pandemic situation has replaced face-to-face teaching and meeting with online teaching and meeting. Recently, the video conferencing tool Zoom has become extremely popular for its simple-to-use feature and low network bandwith requirement. However, Zoom has serious security and privacy issues. Due to weak authentication mechanisms, unauthorized persons are invading Zoom sessions and creating disturbances (known as Zoom bombing). In this paper, we propose a preliminary work towards a seamless authentication mechanism for Zoom-based teaching and meeting. Our method is based on PRNU (Photo Response Non Uniformity)-based camera authentication, which can authenticate the camera of a device used in a Zoom meeting without requiring any assistance from the participants (e.g., needing the participant to provide biometric). Results from a small-scale experiment validates the proposed method.

==> setup/macros.tex <==
%------------------------Custom Commands----------------------%

% = = = Latin Short-forms (ie, eg, etc, et al)
\usepackage{xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\supra}{\textit{Supra}\xspace}
\newcommand{\aka}{\textit{a.k.a.}\xspace}
% \mathchardef\-="2D
\mathchardef\mhyphen="2D


% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}


% = = = Arrow -> (\lt)
\newcommand{\lt}{$\rightarrow$\xspace}
\newcommand{\framework}{\textsl{\mbox{PANDORA}}\xspace}

% = = = Keywords (kw)
\newcommand{\kw}[1]{\textsf{#1}}

% = = = Colored text (textblue)
\newcommand{\textblue}[1]{\textcolor{blue}{#1}}
\newcommand{\textred}[1]{\textcolor{red}{#1}}

% = = = Compact Lists (compactlist, compactlistn)
\newenvironment{compactlist}
  {\begin{itemize}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}}
  {\end{itemize}}

\newenvironment{compactlistn}
  {\begin{enumerate}
  \setlength{\itemsep}{0pt}
  \setlength{\parskip}{0pt}}
  {\end{enumerate}}

\renewcommand{\labelitemi}{$\bullet$}

\newcommand{\pparagraph}[1]{\medskip \noindent \textbf{#1\ }}
\renewcommand{\paragraph}[1]{\medskip \noindent \textbf{#1.\ }}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\iffalse
\newtheorem{mydef}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{proof}{Proof}
\newcommand*{\QEDA}{\hfill\ensuremath{\blacksquare}}
\fi

\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}


==> setup/packages.tex <==
\usepackage{wrapfig}
\usepackage{amsmath}
\usepackage{mathptmx}       % selects Times Roman as basic font
\usepackage{helvet}         % selects Helvetica as sans-serif font
\usepackage{courier}        % selects Courier as typewriter font
\usepackage{type1cm}        % activate if the above 3 fonts are
                            % not available on your system
\usepackage{makeidx}         % allows index generation
\usepackage{graphicx,subfigure}        % standard LaTeX graphics tool
                             % when including figure files
\usepackage{multicol}        % used for the two-column index
\usepackage[bottom]{footmisc}% places footnotes at page bottom
\usepackage{marvosym}
\usepackage{epstopdf}
\usepackage{epsfig}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
%\usepackage{subcaption}
\usepackage{amssymb}         % used for checkmark and times
\usepackage{wasysym}         % used for checkmark and times
%\usepackage{amsthm}
%\usepackage{dingbat}
\usepackage{diagbox}
\usepackage{subfigure}
\usepackage{cite}
\usepackage[hyphens]{url}
\usepackage{hyperref}
\usepackage{breakurl}
\usepackage{dsfont}
\usepackage{todonotes}
\usepackage{color}
%\usepackage{makecell}
\usepackage{caption}

